Bilinear Kloosterman sums in function fields and the distribution of irreducible polynomials

Inspired by the work of Bourgain and Garaev (2013), we provide new bounds for certain weighted bilinear Kloosterman sums in polynomial rings over a finite field. As an application, we build upon and extend some results of Sawin and Shusterman (2022). These results include bounds for exponential sums weighted by the M\"obius function and a level of distribution for irreducible polynomials beyond 1/2, with arbitrary composite modulus. Additionally, we can do better when averaging over the modulus, to give an analogue of the Bombieri-Vinogradov Theorem with a level of distribution even further beyond 1/2.

==> Files/averaging.tex <==
\newpage


Let 
$$S = \sum_{\deg h < k-d}\sum_{\deg x < B}\sum_{\deg y < k-B}\alpha_x\beta_ye_F(a\ov{xy}).$$

Then we have bounds 

$$S \ll q^{2k-d}\left( E^\inv_{F,k_1}(B)E^\inv_{F,k_2}(k-B)q^{r-2Bk_1-2(k-B)k_2}\right)^{1/2k_1k_2}$$

$$S\ll q^{2k-d}\left( E^\mult_F(k-d, B)E_{F,2}^\inv(k-B)q^{r-2(k-d)-2B-4(k-B)}\right)^{1/4}$$

$$S \ll q^{k-d + 3B/4 + r/4}E_{F,2}^\inv(k-B)^{1/4}$$

\newpage 

Let 
$$S = \sum_{\deg z < h}\left|\sum_{\deg x < m}\sum_{\deg y < n}\alpha_x\beta_ye_F(az\ov{xy} )\right|.$$
Applying the triangle inequality and then the Cauchy-Schwarz inequality yields
\begin{align*}
    S^2
    &\leq q^{h+m}\sum_{\deg z < h}\sum_{\deg x < m}\left|\sum_{\deg y < n}\beta_ye_F(az\ov{xy}) \right|^2\\
    &= q^{h+m}\sum_{\deg z < h}\sum_{\deg x < m}\sum_{\deg y_1, y_2 < n}\beta_{y_1}\ov{\beta_{y_2}}e_F(az\ov{x}(\ov{y_1}-\ov{y_2})\\
    &\leq q^{h+m}\sum_{\deg x < m}\sum_{\deg y_1, y_2 < n}\left|\sum_{\deg z < h}e_F(az\ov{x}(\ov{y_1}-\ov{y_2})\right|\\
    &= q^{2h+m}\sum_{\substack{\deg x < m \\\deg y_1, y_2 < n \\ \deg_F(a\ov{x}(\ov{y_1}-\ov{y_2})) < r-h}}1. 
\end{align*}
Thus it suffices to bound the number of solutions to 
$$\ov{y_1}-\ov{y_2} \equiv\ov{a}x_1x_2 \Mod{F}, ~\deg y_i < n, \deg x_1 < m, \deg x_2 < r-h. $$
We write this as
$$\sum_{\deg f < r}I_{F,f}(n)H_{F, af}(m, r-h). $$

We can bring out the hyperbola and take a maximum, to yields 
\begin{align*}
    \sum_{\deg f < r}I_{F,f}(n)H_{F, af}(m, r-h)
    &\leq \max_{\deg f < r}H_{F, af}(m, r-h)\sum_{\deg f < r}I_{F,f}(n)\\
    &\leq (q^{m+r-h-r} + 1)(q^{2n}). 
\end{align*}
Thus 
$$S^2 \leq q^{2h + m + m+r-h-r+2n} + q^{2h + m + 2n} = q^{h + 2m + 2n }+q^{2h + 2n + m}$$
so
$S\leq q^{m+n+h/2} + q^{h+n+m/2}$

OR

We can bring out the inverse and take a maximum, to yields 
\begin{align*}
    \sum_{\deg f < r}I_{F,f}(n)H_{F, af}(m, r-h)
    &\leq \max_{\deg f < r}I_{F, f}(n)\sum_{\deg f < r}H_{F,af}(m, r-h)\\
    &\leq (q^{3n/2 - r/2} + 1)(q^{m+r-h}). 
\end{align*}
Thus 
$$S^2 \leq q^{h+2m+3n/2+r/2} + q^{r+2m+h}$$

